Optimal Treatment Allocation under Constraints

In optimal policy problems where treatment effects vary at the individual level, optimally allocating treatments to recipients is complex even when potential outcomes are known. We present an algorithm for multi-arm treatment allocation problems that is guaranteed to find the optimal allocation in strongly polynomial time, and which is able to handle arbitrary potential outcomes as well as constraints on treatment requirement and capacity. Further, starting from an arbitrary allocation, we show how to optimally re-allocate treatments in a Pareto-improving manner. To showcase our results, we use data from Danish nurse home visiting for infants. We estimate nurse specific treatment effects for children born 1959-1967 in Copenhagen, comparing nurses against each other. We exploit random assignment of newborn children to nurses within a district to obtain causal estimates of nurse-specific treatment effects using causal machine learning. Using these estimates, and treating the Danish nurse home visiting program as a case of an optimal treatment allocation problem (where a treatment is a nurse), we document room for significant productivity improvements by optimally re-allocating nurses to children. Our estimates suggest that optimal allocation of nurses to children could have improved average yearly earnings by USD 1,815 and length of education by around two months.

==> tables/accs-splits-small-meta-fields.tex <==
                                Babbles &            92.9 &                  97.5 &             61.5 \\
                   Breastfeeding 7 days &            99.4 &                  99.7 &             91.4 \\
                   Care and cleanliness &            96.7 &                  99.0 &             60.8 \\
                                   Date &            97.2 &                  96.8 &             77.5 \\
                 Duration breastfeeding &            97.6 &                  97.9 &             97.3 \\
                   Home economic status &            96.0 &                  97.6 &             46.5 \\
                           Home harmony &            97.7 &                  98.9 &             26.5 \\
                                 In air &            91.7 &                  97.5 &             61.2 \\
                                 Length &            99.0 &                  99.0 &             97.2 \\
                             Lifts head &            92.6 &                  94.9 &             63.4 \\
     Mother daily hours working at home &            88.8 &                  99.5 &             60.7 \\
Mother daily hours working outside home &            93.0 &                  99.5 &             70.8 \\
                 Mother mental capacity &            96.8 &                  97.4 &             40.9 \\
               Mother physical capacity &            97.1 &                  98.1 &             41.6 \\
                  Number of daily meals &            74.5 &                  74.0 &             72.9 \\
                Nursery or kindergarten &            93.9 &                  93.3 &             69.9 \\
                              Nutrition &            96.2 &                  97.0 &             80.2 \\
                                Own bed &            96.0 &                  99.7 &             59.7 \\
                          Birth prior to due date &            99.0 &                  99.5 &             88.4 \\
                  Weeks prior to due date  &            97.3 &                  80.1$^{\ast}$ &             12.5 \\
                                   Sits &            91.9 &                  91.8 &             70.3 \\
                                 Smiles &            93.0 &                  98.0 &             61.5 \\
                                 Weight &            97.8 &                  97.7 &             97.3 \\


==> tables/accs-splits-small-names-first.tex <==
Nurse first name &            95.2 &                  93.6 &             57.0 \\


==> tables/accs-splits-small-names-last.tex <==
Nurse last name &            95.0 &                  93.2 &             57.0 \\


==> tables/average-outcome-by-allocation.tex <==
               Breastfed, 1 mo. &       0.58 &       0.60 &       0.62 & 43,259 \\
               Breastfed, 6 mo. &       0.03 &       0.04 &       0.04 & 31,449 \\
Duration of breastfeeding (mo.) &       2.55 &       2.63 &       2.74 & 33,139 \\
          Avg. inc. 25-50 (DKK) & 275,018.01 & 280,699.60 & 286,100.90 & 50,108 \\
              Share empl. 25-50 &       0.80 &       0.81 &       0.82 & 49,186 \\
                  Yrs. of educ. &      13.83 &      13.92 &      14.00 & 48,916 \\
               Above mand. edu. &       0.76 &       0.77 &       0.79 & 48,916 \\


==> tables/descr-by-nurse-rank-controls.tex <==
       Birth weight (g) & 3,284.49 (536.91) & 3,313.56 (528.39) & 3,334.62 (531.45) & 3,357.27 (515.09) & 76,467 \\
                 Low BW &       0.04 (0.19) &       0.05 (0.21) &       0.05 (0.23) &       0.07 (0.25) & 76,467 \\
      Birth length (cm) &      51.23 (2.47) &      51.37 (2.42) &      51.46 (2.41) &      51.59 (2.32) & 76,257 \\
 Born prior to due date &       0.09 (0.29) &       0.12 (0.32) &       0.13 (0.34) &       0.15 (0.36) & 75,118 \\
Weeks prior to due date &       3.08 (1.62) &       3.32 (1.82) &       3.48 (1.88) &       3.74 (2.06) &  8,619 \\
          Year of birth &   1,961.01 (1.75) &   1,962.88 (2.48) &   1,963.36 (2.46) &   1,964.81 (1.84) & 75,899 \\
               Born 1-3 &       0.08 (0.27) &       0.09 (0.29) &       0.10 (0.30) &       0.12 (0.32) & 75,899 \\
           Child parity &       1.54 (0.72) &       1.60 (0.76) &       1.64 (0.80) &       1.71 (0.86) & 75,184 \\
              Firstborn &       0.49 (0.50) &       0.52 (0.50) &       0.54 (0.50) &       0.58 (0.49) & 75,184 \\
                 Female &       0.46 (0.50) &       0.48 (0.50) &       0.50 (0.50) &       0.52 (0.50) & 75,360 \\
   Mother yrs. of educ. &      10.55 (2.98) &      10.99 (3.05) &      11.36 (3.12) &      11.79 (3.20) & 72,303 \\
    Mother age at birth &      23.97 (4.76) &      24.78 (5.21) &      25.32 (5.42) &      26.14 (5.67) & 75,184 \\
   Father yrs. of educ. &      11.61 (3.34) &      12.06 (3.37) &      12.50 (3.37) &      13.01 (3.37) & 64,494 \\
    Father age at birth &      27.23 (6.31) &      28.00 (6.48) &      28.60 (6.75) &      29.38 (6.86) & 72,087 \\
         Father missing &       0.04 (0.20) &       0.05 (0.23) &       0.07 (0.25) &       0.08 (0.27) & 76,579 \\
        High SES, 1 mo. &       0.02 (0.13) &       0.05 (0.22) &       0.10 (0.31) &       0.31 (0.46) & 49,942 \\


==> tables/descr-by-nurse-rank-outcomes-adult.tex <==
Avg. inc. 25-50 (DKK) & 248,926.10 (156,939.84) & 260,964.34 (162,325.75) & 271,131.54 (161,560.47) & 285,750.18 (166,404.97) & 74,922 \\
    Share empl. 25-50 &             0.76 (0.30) &             0.78 (0.29) &             0.80 (0.27) &             0.82 (0.26) & 74,168 \\
        Yrs. of educ. &            13.34 (2.49) &            13.57 (2.51) &            13.79 (2.55) &            14.08 (2.55) & 74,167 \\
     Above mand. edu. &             0.69 (0.46) &             0.72 (0.45) &             0.75 (0.44) &             0.79 (0.41) & 74,167 \\


==> tables/descr-by-nurse-rank-outcomes-child.tex <==
               Breastfed, 1 mo. & 0.49 (0.50) & 0.56 (0.50) & 0.59 (0.49) & 0.64 (0.48) & 70,452 \\
               Breastfed, 6 mo. & 0.01 (0.09) & 0.02 (0.14) & 0.03 (0.17) & 0.06 (0.23) & 63,670 \\
Duration of breastfeeding (mo.) & 1.81 (2.42) & 2.40 (2.75) & 2.61 (2.94) & 3.01 (3.09) & 64,853 \\


==> tables/descr-controls.tex <==
       Birth weight (g) & 3,326.76 & 527.81 & 76,467 & 0.000 \\
                 Low BW &     0.05 &   0.22 & 76,467 & 0.000 \\
      Birth length (cm) &    51.42 &   2.40 & 76,257 & 0.000 \\
 Born prior to due date &     0.12 &   0.33 & 75,118 & 0.000 \\
Weeks prior to due date &     3.41 &   1.87 &  8,619 & 0.001 \\
          Year of birth & 1,963.12 &   2.53 & 75,899 & 0.000 \\
               Born 1-3 &     0.10 &   0.30 & 75,899 & 0.015 \\
           Child parity &     1.63 &   0.79 & 75,184 & 0.000 \\
              Firstborn &     0.53 &   0.50 & 75,184 & 0.000 \\
                 Female &     0.49 &   0.50 & 75,360 & 0.069 \\
   Mother yrs. of educ. &    11.25 &   3.13 & 72,303 & 0.000 \\
    Mother age at birth &    25.17 &   5.38 & 75,184 & 0.000 \\
   Father yrs. of educ. &    12.37 &   3.40 & 64,494 & 0.000 \\
    Father age at birth &    28.41 &   6.67 & 72,087 & 0.000 \\
         Father missing &     0.06 &   0.23 & 76,579 & 0.000 \\
        High SES, 1 mo. &     0.12 &   0.32 & 49,942 & 0.000 \\


==> tables/descr-outcomes-adult.tex <==
Avg. inc. 25-50 (DKK) & 269,452.55 & 162,909.39 & 74,922 &  0.0 \\
    Share empl. 25-50 &       0.79 &       0.28 & 74,168 &  0.0 \\
        Yrs. of educ. &      13.74 &       2.54 & 74,167 &  0.0 \\
     Above mand. edu. &       0.74 &       0.44 & 74,167 &  0.0 \\

==> tables/descr-outcomes-child.tex <==
               Breastfed, 1 mo. & 0.58 & 0.49 & 70,452 &  0.0 \\
               Breastfed, 6 mo. & 0.03 & 0.17 & 63,670 &  0.0 \\
Duration of breastfeeding (mo.) & 2.50 & 2.86 & 64,853 &  0.0 \\


==> tables/mh-models-diff.tex <==
Date       &        date &     67x181 &            3 &       1024 \\
First name &  nurse-name &     91x530 &           18 &        256 \\
Weight     &      weight &     80x258 &            5 &       1024 \\


==> tables/s2s-models-diff.tex <==
Circle       &                                   breastfeed-7-do, birth prior to due date &    100x350 &            4 &        256 \\
Integer seq. &  dura-any-breastfeed, length, weeks prior to due date, tab-b, weight &     90x230 &            7 &       1024 \\
Last name    &                                                       nurse-name &     91x530 &           20 &        512 \\


==> tables/treatment-effects-counterfactuals.tex <==
                 Low BW & 0.03 &  0.00 & 0.05 & 0.119 \\
 Born prior to due date & 0.06 &  0.01 & 0.12 & 0.000 \\
Weeks prior to due date & 0.56 &  0.03 & 3.41 & 0.290 \\
               Born 1-3 & 0.05 &  0.00 & 0.10 & 0.252 \\
                 Female & 0.07 & -0.00 & 0.49 & 0.924 \\
         Father missing & 0.03 & -0.00 & 0.06 & 0.924 \\


==> tables/treatment-effects-dy.tex <==
               Breastfed, 1 mo. &      0.08 &     0.01 &       0.56 & 0.141 \\
               Breastfed, 6 mo. &      0.03 &     0.00 &       0.03 & 0.087 \\
Duration of breastfeeding (mo.) &      0.52 &     0.09 &       2.39 & 0.012 \\
          Avg. inc. 25-50 (DKK) & 28,080.40 & 4,449.58 & 274,341.07 & 0.036 \\
              Share empl. 25-50 &      0.05 &     0.01 &       0.80 & 0.015 \\
                  Yrs. of educ. &      0.45 &     0.09 &      13.80 & 0.007 \\
               Above mand. edu. &      0.07 &     0.01 &       0.76 & 0.141 \\


==> tables/treatment-effects-firstborn.tex <==
               Breastfed, 1 mo. &      0.10 &     0.01 &       0.61 & 0.020 \\
               Breastfed, 6 mo. &      0.03 &     0.00 &       0.03 & 0.059 \\
Duration of breastfeeding (mo.) &      0.65 &     0.13 &       2.59 & 0.000 \\
          Avg. inc. 25-50 (DKK) & 31,249.23 & 1,927.78 & 278,822.14 & 0.090 \\
              Share empl. 25-50 &      0.05 &     0.00 &       0.80 & 0.114 \\
                  Yrs. of educ. &      0.51 &     0.06 &      13.98 & 0.012 \\
               Above mand. edu. &      0.08 &     0.01 &       0.77 & 0.039 \\


==> tables/treatment-effects-mr3.tex <==
               Breastfed, 1 mo. &      0.09 &     0.02 &       0.58 & 0.000 \\
               Breastfed, 6 mo. &      0.03 &     0.00 &       0.03 & 0.003 \\
Duration of breastfeeding (mo.) &      0.59 &     0.15 &       2.50 & 0.000 \\
          Avg. inc. 25-50 (DKK) & 27,965.44 & 4,221.04 & 269,780.38 & 0.000 \\
              Share empl. 25-50 &      0.05 &     0.01 &       0.79 & 0.004 \\
                  Yrs. of educ. &      0.46 &     0.09 &      13.74 & 0.000 \\
               Above mand. edu. &      0.07 &     0.01 &       0.74 & 0.009 \\


==> tables/treatment-effects.tex <==
               Breastfed, 1 mo. &      0.09 &     0.02 &       0.58 & 0.000 \\
               Breastfed, 6 mo. &      0.03 &     0.00 &       0.03 & 0.004 \\
Duration of breastfeeding (mo.) &      0.59 &     0.14 &       2.50 & 0.000 \\
          Avg. inc. 25-50 (DKK) & 27,722.42 & 3,767.50 & 269,452.55 & 0.000 \\
              Share empl. 25-50 &      0.05 &     0.01 &       0.79 & 0.000 \\
                  Yrs. of educ. &      0.47 &     0.09 &      13.74 & 0.000 \\
               Above mand. edu. &      0.07 &     0.01 &       0.74 & 0.006 \\


==> tables/visit-content-1yr.tex <==
                   Family  &                                              Socioeconomic status, mother mental and physical health &             &                  \checkmark &  \checkmark \\
        Mother labor force &                                           Employment status, childcare status &             &                  \checkmark &  \checkmark \\
                 Nutrition &                                                                                                            &             &                             &             \\
            \hspace{3mm}a. &                                                             Infant feeding, number of meals &  \checkmark &                  \checkmark &  \checkmark \\
            \hspace{3mm}b. &                                                                                   Duration of breastfeeding &             &                             &  \checkmark \\        Child development &                                                                                                            &             &                             &             \\
            \hspace{3mm}a. &                                                                    Smiles, lifts head, babbles, sits alone &             &                  \checkmark &  \checkmark \\
            \hspace{3mm}b. &                                                                                                     Height &             &                             &  \checkmark \\
            \hspace{3mm}c. &                                                                                                     Weight &  \checkmark &                  \checkmark &  \checkmark \\
            \hspace{3mm}d. &  Walks, \#teeth, general health assessment, vaccination status, ever hospitalized &             &                             &  \checkmark \\
 
 Child sleeping conditions &                                                                                            Own bed &             &                  \checkmark &  \checkmark

==> tables/visit-content-23yr.tex <==
 Health care take-up &                       GP consultation, dentist visits, vaccinations, diagnosed illnesses &  \checkmark &  \checkmark &  \checkmark &  \checkmark &  \checkmark \\
                       Nutrition &                                                   Vitamins, candy, teeth brushing &  \checkmark &             &  \checkmark &             &  \checkmark \\
                       Illnesses &  Dyspepsia, lung illnesses, otitis, other, accidents &  \checkmark &  \checkmark &  \checkmark &  \checkmark &  \checkmark \\
                 Social development &                           Emotional problems, habit formation &             &  \checkmark &             &  \checkmark &  \checkmark \\
       Parenting style, daycare &                                                                          Strict, parent-child relation &             &             &   &             &  \checkmark \\ 
       Child sleeping conditions &                                                                          Own bed &             &             &  \checkmark &             &  \checkmark
